Space Efficient Deterministic Approximation of String Measures

We study approximation algorithms for the following three string measures that are widely used in practice: edit distance (ED), longest common subsequence (LCS), and longest increasing sequence (LIS). All three problems can be solved exactly by standard algorithms that run in polynomial time with roughly $\Theta(n)$ space, where $n$ is the input length, and our goal is to design deterministic approximation algorithms that run in polynomial time with significantly smaller space. Towards this, we design several algorithms that achieve $1+\epsilon$ or $1-\epsilon$ approximation for all three problems, where $\epsilon>0$ can be any constant and even slightly sub constant. Our algorithms are flexible and can be adjusted to achieve the following two regimes of parameters: 1) space $n^\delta$ for any constant $\delta>0$ with running time essentially the same as or slightly more than the standard algorithms; and 2) space $\mathsf{polylog}(n)$ with (a larger) polynomial running time, which puts the approximation versions of the three problems in Steve's class (\textbf{SC}). Our algorithms significantly improve previous results in terms of space complexity, where all known results need to use space at least $\Omega(\sqrt{n})$. Some of our algorithms can also be adapted to work in the asymmetric streaming model [SS13], and output the corresponding sequence. Furthermore, our results can be used to improve a recent result by Farhadi et. al. [FHRS20] about approximating ED in the asymmetric streaming model, reducing the running time from being exponential in [FHRS20] to a polynomial. Our algorithms are based on the idea of using recursion as in Savitch's theorem [Sav70], and a careful adaption of previous techniques to make the recursion work. Along the way we also give a new logspace reduction from longest common subsequence to longest increasing sequence, which may be of independent interest.

==> ed_polylog.tex <==
\section{Edit distance}



We now present our algorithm that gives a $(1+o(1))$-approximation with only polylogarithmic space. We first introduce a massively parallel algorithm from \cite{hajiaghayi2019massively}

\subsection{Massively parallel algorithm for edit distance}

To make this work complete and self-contained, we first introduce the ideas from \cite{hijiaghayi2019massively}...

Let $x$ and $y$ be two strings with $|x|=n$ and $|y| = m$. Our goal is to output a $1+\eps$ approximation for $\ed(x,y)$. Here, $\eps$ can be subconstant (In our main algorithm, we pick $\eps$ to be $O(\frac{1}{\log n})$). In our algorithm, we only consider the case when $n = \Theta(m)$ since otherwise output a good approximation of $\ed(x,y)$ would be easy. 

We assume a value $\Delta$ is given to us which is supposed to be a $1+\eps$ approximation of the actual edit distance. Such an assumption only increase the total amount of computation by a $O(\log_{1+\eps}(n))$ \cite{boroujeni2018approximating}. This is because we can try all $\Delta = (1+\eps)^i$ with $i\in [\rceil \log_{1+\eps}(n)\rceil] $ and make sure one of $\Delta$ is a $1+\eps$ approximaition of $\ed(x,y)$.

Given such a $\Delta$, we first divide string $x$ into $b$ blocks ($b$ is a parameter we will pick later). We denote the $i$-th block by $x^i$. Then for each block, say $x^i$, we determine a set of substrings of $y$ as candidate intervals such that one of the candidate substrings is close to the optimal substring $x^i$ is matched to in the optimal matching. We call such a substring \emph{approximately optimal candidate}. Then, if we know the edit distance (or a good approximation of edit distance) between each block and each of its candidate substring of $y$, we can run a dynamic programming to get a approximation of the actual distance. 


%We first divide $x$ into $N = n^\delta$ blocks  each of size at most $\lceil n/N\rceil $ and write $x$ as $x^1\circ x^2 \circ \cdots \circ x^{N}$ where $x^i = x_{[l_i,r_i]}$. That is, $x^i$ starts at the $l_i$-th position and ends at the $r_i$-th position. In the following discussion, we fix an optimal alignment such that $x_{[l_i,r_i]}$ is mapped to a block $y_{[\alpha_i,\beta_i]}$ and $[\alpha_i,\beta_i]$'s are disjoint and span the entire length of $y$. This optimal alignment minimizes the operations needed to transform $x$ into $y$. Then, we give the following definition of \emph{$(\eps,\Delta)$-approximately optimal candidate}.

In the following analysis, we fix an optimal alignment between $x$ and $y$ where the $i$-th block $x_{[l_i,r_i]}$ is matched to substring $y_{[\alpha_i,\beta_i]}$ such that the intervals $[\alpha_i,\beta_i]$'s are disjoint and span the entire length of $y$. By the assumption, we have $\ed(x,y) = \sum_{i = 1}^{N}\ed(x^i,y_{[\alpha_i,\beta_i]})$.

We now give the definition of \emph{$(\eps,\Delta)$-approximately optimal candidate}.

\begin{definition}
	[\cite{hajiaghayi2019massively}]
	\label{approx_optimal_candidate}
	We say an interval $[\alpha',\beta']$ is an \emph{$(\eps,\Delta)$-approximately optimal candidate} of the block $x^i = x_{[l_i,r_i]}$ if the following two conditions hold:
	\[\alpha_i\leq \alpha'\leq \alpha_i+\eps\frac{\Delta}{N}\]
	\[\beta_i-\eps\frac{\Delta}{N}-\eps \ed(x_{[l_i,r_i]},y_{[\alpha_i,\beta_i]})\leq \beta'\leq \beta_i\]
\end{definition}

We first show that if $\Delta$ is a good approximation of $\ed(x,y)$, and for each block that is not matched to a too large or a too small interval, we know the edit distance between it and one of its approximately optimal candidate, we can get a good approximation of $\ed(x,y)$. We put it formally in Lemma~\ref{lem:approx_optimal_candidate}.

\begin{lemma}[Implicit from \cite{hajiaghayi2019massively}]
	\label{lem:approx_optimal_candidate}
	Let $\eps\in (0,1)$ ($\eps $ can be subconstant) and $\eps' = \eps/10$. Assume $\ed(x,y)\leq \Delta\leq (1+\eps')\ed(x,y)$.  For each $i\in [N]$, let $(\alpha_i',\beta_i')$ be any $(\eps',\delta)$-approximately optimal candidate of $x^i$. If $\eps'|\alpha_i-\beta_i+1|\leq |x^i|\leq 1/\eps'|\alpha_i-\beta_i +1|$, let $D'_i =|\alpha_i-\alpha'_i|+ \ed(x^i,y_{[\alpha'_i,\beta'_i]}) + |\beta_i-\beta'_i| $. Otherwise, let $D'_i  = |x^i| + |\alpha_i-\beta_i+1|$. Then
	\[\ed(x,y)\leq \sum_{i = 1}^{N}D'_i \leq (1+\eps)\ed(x,y).\]
\end{lemma}

To make our work self-contained, we provide a proof here.

\begin{proof}[Proof of Lemma~\ref{lem:approx_optimal_candidate}]
	Let $D_i = \ed(x^i,y_{[\alpha_i,\beta_i]})$. Since we assume the alignment is optimal and $[\alpha_i,\beta_i]$ are disjoint and span the entire length of $y$,  we know $\ed(x,y) = \sum_{i = 1}^{N}D_i$. 
	
	For each $i\in [N]$, if $\eps'|\alpha_i-\beta_i+1|\leq |x^i|\leq 1/\eps'|\alpha_i- \beta_i+1|$, by the defition of \emph{$(\eps',\Delta)$-approximately optimal condiate}, we know, 
	\begin{equation}
	\label{a}
	|\alpha_i-\alpha'_i|\leq \eps'\frac{\Delta}{N}
	\end{equation}
	and
	\begin{equation}
	\label{b}
	|\beta_i-\beta'_i| \leq \eps'\frac{\Delta}{N} + \eps' \ed(x^i, y_{[\alpha_i,\beta_i]})
	\end{equation}
	
	Also notice that we can transform  $y_{[\alpha'_i,\beta'_i]}$ to $y_{[\alpha_i,\beta_i]}$ with $|\alpha_i-\alpha'_i|+|\beta_i-\beta'_i| $ insertions and then transform $y_{[\alpha_i,\beta_i]}$ to $x^i$ with $\ed(x^i,y_{[\alpha_i,\beta_i]}) $ edit operations. We have
	\begin{equation}
	\label{c}
	\ed(x^i,y_{[\alpha'_i,\beta'_i]})\leq \ed(x^i,y_{[\alpha_i,\beta_i]}) + |\alpha_i-\alpha'_i|+|\beta_i-\beta'_i|
	\end{equation}
	
	Meanwhile, we can always transform $y_{[\alpha_i,\beta_i]}$ to $y_{[\alpha'_i,\beta'_i]}$ with $|\alpha_i-\alpha'_i|+|\beta_i-\beta'_i| $ deletions and then transform $y_{[\alpha'_i,\beta'_i]}$ to $x^i$ with $\ed(x^i,y_{[\alpha'_i,\beta'_i]})$. We have 
	\begin{equation}
	\label{f}
	D'_i\geq D_i.
	\end{equation}
	
	Combining \ref{a} \ref{b} \ref{c} and \ref{f}, we have
	
	\begin{equation}
	\label{d}
	D_i\leq D'_i\leq \ed(x^i,y_{[\alpha_i,\beta_i]}) + 2|\alpha_i-\alpha'_i|+2|\beta_i-\beta'_i| \leq (1+2\eps')D_i + 4 \eps'\frac{\Delta}{N}.
	\end{equation}
	
    For those $i$ such that $|x^i|>(1/\eps')|\alpha_i-\beta_i+1|$ or $ |x^i|<\eps'|\alpha_i-\beta_i+1|$, to transform $x^i $ to $y_{[\alpha_i,\beta_i]}$, we need to insert (or delete) $||\alpha_i-\beta_i+1|-|x^i||$ characters to make sure the length of $x^i$ equals to the length of $y_{[\alpha_i,\beta_i]}$. Thus, $D_i=\ed (x^i,y_{[\alpha_i,\beta_i]})$ is at least $ ||\alpha_i-\beta_i|-|l_i-r_i||$.  Since $D'_i = |\alpha_i-\beta_i|+|l_i-r_i|$, we have 
	\begin{equation}
	\label{e}
	\begin{aligned}
	D'_i\leq &\frac{1+\eps'}{1-\eps'}D_i &\\
	\leq & (1+3\eps')D_i & \text{Since we set } \eps' = \eps/10\leq 1/10
	\end{aligned}
	\end{equation}
	
	Also notice that we can turn $x^i$ into $y_{[\alpha_i,\beta_i]}$with $|l_i-r_i|$ deletions and $|\alpha_i-\beta_i|$ insertions, we know $D'_i\geq D_i$. It gives us 
	\begin{equation}
	\label{g}
	D_i\leq D'_i\leq (1+3\eps')D_i 
	\end{equation}
	
	Thus for each $i \in [N]$, by \ref{g} and \ref{d}, we have 
	\begin{equation}
	D_i\leq D'_i\leq (1+3\eps') D_i + 4\eps' \frac{\Delta}{N} .
	\end{equation}
	
	Since we assume $ \Delta\leq (1+\eps')\ed(x,y)$, we have $\eps'  \Delta\leq 1.1 \eps'\ed(x,y)$, this gives us 
	\begin{equation}
	\ed(x,y)\leq  \sum_{i = 1}^{N}D'_i  \leq  (1+3\eps') \ed(x,y)+ 4\eps' \Delta\leq (1+10\eps')\ed(x,y) = (1+\eps)\ed(x,y).
	\end{equation}
	
	
\end{proof}

We now show that, for each $i$ and $\eps, \Delta$, without knowing the optimal alignment, we can pick a small set of candidate intervals such that one of the intervals is an \emph{$(\eps , \Delta)$-approximately optimal candidate} for $x^i$.  

That is, there exist a set of intervals $C^i_{\eps,\Delta}$ with size $O(b\log n/\eps^2)$ and one of the intervals in $C^i_{\eps,\Delta}$ is an \emph{$(\eps , \Delta)$-approximately optimal candidate} for $x^i$. The set $C^i_{\eps,\Delta}$ can be find with the algorithm \emph{CandidateSet} which is implicit from \cite{hajiaghayi2019massively}. The algorithm takes six inputs : three integers $n$, $m$, and $b$, an interval $(l_i,r_i)$, $\eps\in (0,1)$, and $\Delta\leq n$ and outputs set $C^i_{\eps,\Delta}$. Here, $n$ and $m$ are the lengths of string $x$ and $y$ correpondingly. The pseudocode is given in algorithm~\ref{algo:CandidateSet}. 

\begin{algorithm}[H]
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{three integers $n$, $m$, and $N$, an interval $(l_i,r_i)$, $\eps\in (0,1)$, and $\Delta\leq n$} 
	$|x^i| = r_i-l_i+1$ \;
	initialize $C$ to be an empty set \;
	
	\ForEach{$i'\in [l_i-\Delta- \eps\frac{ \Delta}{b},l_i+\Delta+  \eps\frac{ \Delta}{b} ]\cap [m]$ such that $i'$ is a multiple of $\lceil \eps \frac{ \Delta}{b}\rceil $ }{
		\Comment{if $\lceil \eps \frac{ \Delta}{b}\rceil=0$, we loop every $i'$ in $[l_i-\Delta-1,l_i+\Delta+1]\cap [m]$}
		
		%\ForEach{$j'\in\{0,1,\lceil 1+\eps\rceil, \lceil (1+\eps)^2\rceil,\cdots,\lceil (1+\eps)^{\lceil \log_{1+\eps}(m)\rceil }\rceil, \text{with no repetition}\}$ }{
		\ForEach{$j'=0 $ \textbf{or} $j' =  \lceil (1+\eps)^i \rceil \textbf{ for some integer } i\leq \lceil \log_{1+\eps}(m)\rceil  \}$ }{
			%%%%% some comment here
			\Comment{pick $O(\log_{1+\eps} n)$ ending points}
			\If{ $|x^i|-j' \geq \eps|x^i| $}{
				add $(i',i'+|x^i|-1-j')$ to $C$ \;
			}
			\If{$|x^i|+j' \leq 1/\eps|x^i| $}{
				add $(i',i'+|x^i|-1+j')$ to $C$ \;
			}
		}	
	}
	\Return{$C$}
	
	\caption{CandidateSet}
	\label{algo:CandidateSet}
\end{algorithm}

\begin{lemma}[Implicit from \cite{hajiaghayi2019massively}]
	\label{lem:CandidateSet}
	If $\eps m\leq n \leq \frac{1}{\eps} m$, then $C^i_{\eps,\Delta} = \text{CandidateSet}(n,m,b,(l_i,r_i),\eps,\Delta)$ is of size $ O(\frac{b\log n}{\eps^2})$. For $x^i = x_{[l_i,r_i]}$, if $\eps|\alpha_i-\beta_i+1|\leq |x^i|\leq 1/\eps|\alpha_i-\beta_i+1|$ and $\Delta\geq \ed(x,y)$, then one of the elements in $C^i_{\eps,\Delta}$ is an \emph{$(\eps, \Delta)$-approximately optimal candidate} of $x^i$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:CandidateSet}]
	Let $C^i_{\eps,\Delta}$ be the output of $\text{CandidateSet}(n,m,b,(l_i,r_i),\eps,\Delta)$. For the starting point $i'$, we only choose multiples of $\eps \frac{ \Delta}{b}$ from $[l_i-\Delta-\eps\frac{ \Delta}{b},l_i+\Delta+\eps\frac{ \Delta}{b}]$. At most $ O(\Delta/(\eps\frac{\Delta}{b}))  = O(b/\eps)$ starting points will be chosen. For each starting point, we consider $O(\log_{1+\eps} m) = O(\frac{\log m}{\eps})= O(\frac{\log n}{\eps})$ ending point since we assume $\eps m\leq n \leq \frac{1}{\eps} m$. Thus, the size of set $C^i_{\eps,\Delta}$ is at most $ O(\frac{b\log n}{\eps^2})$.
	
	We now show there is an element in $C^i_{\eps,\Delta} = \text{CandidateSet}(n,m,b,(l_i,r_i),\eps,\Delta)$ that is an \emph{$(\eps, \Delta)$-approximately optimal candidate} of $x^i$ if $\eps|\alpha_i-\beta_i+1|\leq |x^i|\leq 1/\eps|\alpha_i-\beta_i+1|$. 
	
	Since we assume $\Delta\geq \ed(x,y)$, we are guaranteed that $l_i-\Delta\leq \alpha_i\leq l_i+\Delta$. Thus, there is a multiple of $\lceil\eps \frac{ \Delta}{b}\rceil$, denoted by $\alpha'$, such that
	
	$$l_i-\Delta-\eps\frac{ \Delta}{b}\leq \alpha_i\leq \alpha' \leq \alpha_i+\eps \frac{ \Delta}{b}\leq l_i+\Delta+\eps\frac{ \Delta}{b},$$
	since we try every multiple of $\lceil\eps \frac{ \Delta}{N}\rceil$ between $l_i-\Delta-\eps\frac{ \Delta}{N}$ and $l_i+\Delta+\eps\frac{ \Delta}{N}$, one of them equals to $\alpha'$.
	
	%%%%% 
	For the ending point, we first consider the case when the length of  $y_{[\alpha_i,\beta_i]}$ is larger than the length of $x^i$, that is $\beta_i-\alpha_i+1\geq r_i-l_i+1$. We know $\ed(x^i,y_{[\alpha_i,\beta_i]})\geq \beta_i-\alpha_i+1 -|x^i|$. Let $j$ be the largest element in $\{0,1,\lceil 1+\eps\rceil, \lceil (1+\eps)^2\rceil,\cdots,\lceil (1+\eps)^{\log_{1+\eps}(m)}\rceil\}$ such that $\alpha'+|x^i|-1 +j\leq \beta_i$. We set $\beta' = \alpha'+|x^i|-1+j$. Since $j\geq (\beta_i-(\alpha'+|x^i|-1)/(1+\eps)$, we have
	\begin{equation}
	\begin{aligned}
	\beta' \geq& \alpha'+|x^i|-1+(\beta_i-(\alpha'+|x^i|-1))/(1+\eps)\\
	\geq & \frac{\beta_i}{1+\eps}+\frac{\eps}{1+\eps}(\alpha'+|x^i|-1)\\
	\geq & \beta_i - \frac{\eps}{1+\eps} (\beta_i-\alpha'+1-|x^i|)\\
	\geq &\beta_i - \eps \ed(x^i,y_{[\alpha_i,\beta_i]})
	\end{aligned}
	\end{equation}
	
	The last inequality is because $\ed(x^i,y_{[\alpha_i,\beta_i]})\geq \beta_i-\alpha_i+1-|x^i|\geq \beta_i-\alpha'+1-|x^i|$ and $\eps \geq \frac{\eps}{1+\eps} $. Thus, $(\alpha', \beta')\in C^i_{\eps,\Delta}$ is an \emph{$(\eps, \Delta)$-approximately optimal candidate} of $x^i$. 
	
	For the case when $\beta_i - \alpha_i + 1< |x^i|$. Similarly, we know $\ed(x^i,y_{[\alpha_i,\beta_i]})\geq  |x^i|-(\beta_i-\alpha_i+1)$.We pick $j$ to be the smallest element in $\{0,1,\lceil 1+\eps\rceil, \lceil (1+\eps)^2\rceil,\cdots,\lceil (1+\eps)^{\log_{1+\eps}(m)}\rceil\}$ such that $\alpha'+|x^i|-1-j\leq \beta_i$. We know $j\leq (1+\eps) (\alpha'+|x^i|-1-\beta_i)$. We set $\beta' = \alpha'+|x^i|-j$. Then
	\begin{equation}
	\begin{aligned}
	\beta' \geq& \alpha'+|x^i|-1-(1+\eps)(\alpha'+|x^i|-1-\beta_i)\\
	\geq & \beta_i-\eps(\alpha'-\beta_i+|x^i|-1)\\
	\geq & \beta_i - \eps(\alpha_i+\eps\frac{\Delta}{N}-\beta_i+|x^i|-1)\\
	\geq &\beta_i - \eps \ed(x^i,y_{[\alpha_i,\beta_i]})-\eps^2\frac{\Delta}{N}\\
	\geq &\beta_i - \eps \ed(x^i,y_{[\alpha_i,\beta_i]})-\eps\frac{\Delta}{N}
	\end{aligned}
	\end{equation}
	Thus, $(\alpha', \beta')\in C^i_{\eps,\Delta}$ is an \emph{$(\eps, \Delta)$-approximately optimal candidate} of $x^i$. 
	
\end{proof}

%We now describe a dynamic programming algorithm \emph{DPEditDistance} that computes an approximation of $\ed(x,y)$ with the information of edit distances between $x^i$ and each of intervals in $C^i_{\eps,\Delta}$. \emph{DPEditDistance} takes six inputs, $n$, $m$, $N$, $\Delta$, $\eps$, and a two dimensional list $M$ such that $M(i, (\alpha,\beta)) = \ed(x^i, y_{[\alpha, \beta]})$ for each $i$ and $(\alpha,\beta)\in  C^i_{\eps,\Delta}$. The pseudocode is given in algorithm~\ref{algo:DPEditDistance}.

Given the information of edit distances between $x^i$ and each of intervals in $C^i_{\eps,\Delta}$, we can run a simple dynamic programming algorithm \emph{DPEditDistance} to get an approximation of $\ed(x,y)$.  \emph{DPEditDistance} takes six inputs, $n$, $m$, $b$, $\Delta$, $\eps$, and a two dimensional list $M$ such that $M(i, (\alpha,\beta)) = \ed(x^i, y_{[\alpha, \beta]})$ for each $i$ and $(\alpha,\beta)\in  C^i_{\eps,\Delta}$. The pseudocode is given in algorithm~\ref{algo:DPEditDistance}. 


\begin{algorithm}[H]
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{three integers $n$, $m$, $b$, $\Delta\leq n$, $\eps\in (0,1)$, and a two dimensional list $M$ such that $M(i, (\alpha,\beta)) = \ed(x^i, y_{[\alpha, \beta]})$ for each $i$ and $(\alpha,\beta)\in  C^i_{\eps,\Delta}$.} 
	let $C^i$ be the set of starting points of intervals in $C^{i}_{\eps,\Delta}$ with no repetition for each $i\in [N]$ \;

	\ForEach{$\alpha\in C^1$ }{
		$A(0,\alpha-1) = \alpha-1$ \Comment{$A$ is a two dimensional array for storing the intermediate results of the dynamic programming }\;
	}
	\For{$i=1$ \textbf{to} $b-1$}{
		\ForEach{ $\alpha\in C^{i+1}$  }{
			\(A(i,\alpha-1) = \min \begin{dcases}
			\min_{\alpha'\in C^i, \alpha'\leq \alpha}A(i-1,\alpha'-1)+ |\alpha-\alpha'| +|x^i|\\
			\min_{ \substack{(\alpha',\beta')\in C^i_{\eps,\Delta} \\\text{s.t. } \beta' \leq \alpha-1} }A(i-1,\alpha'-1)+M(i,(\alpha',\beta')) + \alpha-1-\beta'\\
			\end{dcases}
			\) \label{algo:DPEditDistance_updating}\;
		}
	}
	
	\(d = \min
	\begin{dcases}
	\min_{\alpha'\in C^{b}}A(b-1,\alpha'-1)+ |m-\alpha'| + |x^b|\\
	\min_{ \substack{(\alpha',\beta')\in C^b_{\eps,\Delta} \\\text{s.t. } \beta' \leq m} }A(b-1,\alpha'-1)+M(b,(\alpha',\beta')) + m-\beta'\\
	\end{dcases}
	\)\label{DPEditDistance:last}\;
	\Return d
	\caption{DPEditDistance}
	\label{algo:DPEditDistance}
\end{algorithm}



\begin{lemma}
	\label{lem:DPEditDistance}
	For any fixed $\eps$, we let $\eps' = \eps/10$. Assume $\ed(x,y)\leq \Delta\leq (1+\eps')\ed(x,y)$ and $\ed(x^i,y_{[\alpha,\beta]})= M(i,(\alpha,\beta))$, then $\text{DPEditDistance}(n,m,b, \eps',\Delta,M)$ outputs a $(1+\eps)$-approximation of $\ed(x,y)$ in $O(\frac{b^3\log n}{\eps^3})$ time with $O(\frac{b}{\eps}\log n)$ bits of space. 
	
	Also, in the input, if we replace $M(i,(\alpha,\beta))$ with a $(1+\gamma)$ approximation of $\ed(x^i,y_{[\alpha,\beta]})$, that is \[\ed(x^i,y_{[\alpha,\beta]})\leq M(i,(\alpha,\beta))\leq (1+\gamma)\ed(x^i,y_{[\alpha,\beta]})\]
	then $\text{DPEditDistance}(n,m,N, \eps',\Delta,M)$ outputs a $(1+\eps)(1+\gamma)$-approximation of $\ed(x,y)$.
\end{lemma}
\begin{proof}[Proof of Lemma~\ref{lem:DPEditDistance}]
	%Our goal is to find an optimal matching between each block and its candadite set. 
	We start by explaining the dynamic programming. Let $f$ be a function such that $f(i)\in C^i_{\eps',\Delta} \cup \{\emptyset\}$. We say an interval $x^i$ is matched if $f(i)\in C^i_{\eps',\Delta}$ and it is unmatched if $f(i) = \emptyset$. Let $S^f_1$ be the set of indices of matched blocks under function $f$ and $S^f_2 = [N]\setminus S^f_1$ be the set of indices of unmatched blocks. We let $f(i) = (\alpha^f_i,\beta^f_i)$ for each $i\in S^f_1$. We also require that,  for any $i,j\in S^f_1$ with $i<j$, $(\alpha^f_i,\beta^f_i)$ and $(\alpha^f_j,\beta^f_j)$ are disjoint and $\beta^f_i<\alpha^f_j$. Let $u_f$ be the number of unmatched characters under $f$ in $x$ and $y$. That is, $u_f$ equals to the number of indices in $[n]$ that is not in any matched block plus the number of indices in $[m]$ that is not in $f(i)$ for any $i\in S^f_1$.  Then we define the edit distance under match $f$ by \[\ed_f \coloneqq \sum_{i\in S^f_1}\ed(x^i, y_{[\alpha^f_i,\beta^f_i]})+u_f.\]
	
	Since we can always transform $x$ to $y$ by deleting (inserting) every unmatched characters in $x$ ($y$), and transforming each matched block $x^i$ into $y_{[\alpha^f_i,\beta^f_i]}$ with $\ed(x^i, y_{[\alpha^f_i,\beta^f_i]})$ edit operations. We know $\ed_f\geq \ed(x,y)$ 
	
	Let $F$ be the set of all matchings. Also, given $i\in [b]$ and $\alpha\in [m]$, we let $F^{i,\alpha}$ be the set of matching such that $f(i')$ is within $(1,\alpha)$ for all $i'\leq i$. Similarly, for each $f\in F^{i,\alpha}$, let $u^{i,\alpha}_f$ be the number of unmatched characters in $x_{[1,r_i]}$ and $y_{[1,\alpha]}$ under $f$. We can also define $\ed^{i,\alpha}_f = \sum_{i\in S^f_1}\ed(x^i, y_{[\alpha^f_i,\beta^f_i]})+u^{i,\alpha}_f$. For simplicity, let $C^i$ be the set of starting points of all intervals in $C^{i+1}_{\eps,\Delta}$. We now show that in algorithm~\ref{algo:DPEditDistance}, for each $i\in[b-1]$ and $\alpha\in C^{i+1}$, we have 
	
	\[A(i,\alpha-1) = \min_{f\in F^{i,\alpha-1}}\ed^{i,\alpha-1}_f.\] 
	
	We can proof this by induction on $i$. For the base case $i = 1$, we fix an $\alpha\in C^{2}$. For each $f\in F^{1,\alpha-1}$, if $f(1) = \emptyset$, then every character in $x^1$ and $y_{[1,\alpha-1]}$ are unmatched. In this case, $\ed^{1,\alpha-1}_f = |x^1|+\alpha -1 = A(0,\alpha'-1) + \alpha-\alpha' +|x^1|$ for every $\alpha'\in C^1$ such that $\alpha'\leq \alpha$. When $f(1) \neq \emptyset$, we assume $f(1) = (\alpha^f_1,\beta^f_1)$, then $\ed^{i,\alpha-1}_f = \alpha^f_1-1 + M(1,(\alpha^f_i,\beta^f_i))+ \alpha -\beta = A(0,\alpha^f)+ M(1,(\alpha^f_i,\beta^f_i))+ \alpha -\beta $. By the updating rule of $A(1,\alpha-1)$ at line~\ref{algo:DPEditDistance_updating}, we know $A(1,\alpha-1) = \min_{f\in F^{1,\alpha-1}}\ed^{1,\alpha-1}_f$ for every $\alpha\in C^{2}$.
	
	Now assume $A(t-1,\alpha-1) = \min_{f\in F^{t-1,\alpha-1}}\ed^{t-1,\alpha-1}_f$ for any $\alpha\in C^{t}$ for $1<t\leq b-1$. Fix an $\alpha_0\in C^{t+1}$, we show $A(t,\alpha_0-1) = \min_{f\in F^{t,\alpha_0-1}}\ed^{t,\alpha_0-1}_f$. For each matching $f$, if $f(t) = \emptyset$, we know 
	\[\ed^{t,\alpha_0-1}_f = \ed^{t-1,\alpha_0-1}_f + |x^t| \geq \min_{\alpha'\in C^{t},\alpha'\leq \alpha}A(t-1,\alpha'-1)+ \alpha_0-\alpha'\geq A(t,\alpha_0-1).\]
	When $f(t)\neq \emptyset$, we assume $f(t) = (\alpha^f_t,\beta^f_t)$. Then 
	\begin{align*}
	\ed^{t,\alpha_0-1}_f &= \ed^{t-1,\alpha^f_t-1}_f + M(t,(\alpha^f_t,\beta^f_t)) + \alpha_0-\beta^f_t-1\\
	& \geq A(t-1,\alpha^f_t-1)+M(t,(\alpha^f_t,\beta^f_t)) + \alpha_0-\beta^f_t-1\\
	&\geq A(t,\alpha_0-1)
	\end{align*}
	Meanwhile, $A(t,\alpha_0) \geq \min_{f\in F^{t,\alpha_0-1}}\ed^{t,\alpha_0-1}_f$ since $A(t,\alpha_0) = \ed^{t,\alpha_0-1}_f$ for some $f\in F^{t,\alpha_0-1}$ by the updating rule at line~\ref{algo:DPEditDistance_updating}. Thus, we have proved  $A(t,\alpha_0-1) = \min_{f\in F^{t,\alpha_0-1}}\ed^{t,\alpha_0-1}_f$.
	Now, assume we have computed $A(b-1,\alpha)$ for every $\alpha\in C^{b}$. Let $f_0$ be the optimal matching such that $\ed_{f_0}(x,y) = \min_{f\in F} \ed_f(x,y)$.  If $f_0(b) = \emptyset$, 
	\[\ed_{f_0}(x,y) = \min_{\alpha'\in C^{b}}A(b-1,\alpha'-1)+ |m-\alpha'| + |x^b|\]
	Otherwise, let $f_0(b) = (\alpha^{f_0}_b,\beta^{f_0}_b)$
	\[\ed_{f_0}(x,y)  = \min_{ (\alpha',\beta')\in C^b_{\eps,\Delta}}A(b-1,\alpha'-1)+M(b,(\alpha^{f_0}_b,\beta^{f_0}_b)) + m-\beta'\]
	By the optimality of $f_0$, we know the algorithm~\ref{algo:DPEditDistance} is $d = \ed_{f_0}(x,y)$. Now, if we fix an optimal alignment such that $x_{[l_i,r_i]}$ is matched  to block $y_{[\alpha_i,\beta_i]}$ and $[\alpha_i,\beta_i]$ are disjoint and span the entire length of $y$. Let $f_1$ be a matching such that, for each $i\in [b]$, if $\eps'|\alpha_i-\beta_i|\leq |l_i-r_i|\leq 1/\eps'|\alpha_i-\beta_i|$, $f(i)$ is an \emph{$(\eps', \Delta)$-approximately optimal candidate}. Otherwise, $f(i) = \emptyset$. By lemma~\ref{lem:approx_optimal_candidate} and lemma~\ref{lem:CandidateSet}, such a matching $f_1$ exists and $\ed_f\leq (1+\eps)\ed(x,y)$. Thus,
	\[\ed(x,y)\leq\ed_{f_0}\leq \ed_{f_1}\leq (1+\eps)\ed(x,y)\]
	This proves the correctness of algorithm~\ref{algo:DPEditDistance}. 
	
	Now we compute the tme complexity. By the proof of lemma~\ref{lem:CandidateSet}, $|C^i| = O(\frac{b}{\eps})$ for $i\in [b]$. The size of matrix $A$ is $O(\frac{b^2}{\eps})$ where the rows of $A$ are indexed by $i$ from $0$ to $b-1$ and for the $i$-th row, the columns are indexed by the elements in set $C^{i+1}$. We can divide the dynamic programming into roughly $b$ steps and for the $i$-th step, we compute the row indexed by $i$.  Assume we have already computed the row indexed by $i-1$ of $A$. We first set 
	$$A(i,\alpha-1) = \min_{\alpha'\in C^i,\alpha'\leq \alpha} A(i-1,\alpha'-1) + \alpha-\alpha'+ |x^i|$$
	for all $\alpha \in C^i$. This takes $O(|C^i||C^{i+1}|) = O(\frac{b^2}{\log^2 n})$ time. Then, we query each elements in the $i$-th row of $M$. Say we queried $M(i, (\alpha',\beta'))$, we update all $A(i,\alpha-1)$ such that $\alpha-1\geq \beta'$ by 
	$$A(i,\alpha-1) = \min\{A(i,\alpha-1),A(i-1,\alpha'-1)+M(i,(\alpha',\beta')) + \alpha-1 -\beta'\}.$$
	This takes $O(|C^i_{\eps', \Delta}||C^{i+1}|) = O(\frac{b^2}{\eps^3}\log n)$ time. So the $i$-th step takes $O(\frac{b^2}{\eps^3}\log n)$ time. SInce there are $b$ steps, the time complexity is bound by $O(\frac{b^3}{\eps^3}\log n)$.
	
	%For computing each $A(i,\alpha-1)$, we take the minimum over every $(\alpha',\beta')\in C^i_{\eps', \Delta}$. By Lemma~\ref{lem:CandidateSet}, the size of $C^i_{\eps', \Delta}$ is at most $O(\frac{b \log n}{\eps^2})$. This takes at most $O(\frac{b \log n}{\eps^2})$ time. Thus, everything before line~\ref{DPEditDistance:last} takes $O(\frac{b^3 \log n}{\eps^3})$ time. For line~\ref{DPEditDistance:last}, we take the minimum over every $(\alpha',\beta')\in C^b_{\eps', \Delta}$, this again takes $O(\frac{b \log n}{\eps^2})$ time. The total time required is $O(\frac{b^3 \log n}{\eps^3})$. 
	
	For the space complexity, notice when updating $A(i,\alpha)$, we only need the information of $A(i-1, \alpha'-1)$ for every $\alpha'\in C^i$. Thus, we can release the space used to store $A(i-2, \alpha''-1)$ for every $\alpha''\in C^{i-1}$. And for line~\ref{DPEditDistance:last}, we only need the information of $A(i-1, \alpha-1)$ for every $\alpha\in C^b$. From algorithm~\ref{algo:CandidateSet}, we know that for each $i$, we pick at most $ b/\eps$ points as the starting point of the candidate intervals. The size of  $C^b$ is at most $b/\eps$. Since each element in $A$ is a number at most $n$, it can be stored with $O(\log n)$ bits of space. Thus, the space required is $O(\frac{b}{\eps}\log n)$.
	
	If we replace $M(i,(\alpha,\beta))$ with a $(1+\gamma)$ approximation of $\ed(x^i,y_{[\alpha,\beta]})$. Each $M(i,(\alpha,\beta))$ will add at most an $\gamma\ed(x^i,y_{[\alpha,\beta]})$ additive error. The amount of error added is bounded by $\gamma \ed(x,y)$. Thus, $\text{DPEditDistance}(n,m,b, \eps',\Delta,M)$ outputs a $(1+\eps)(1+\gamma)$-approximation of $\ed(x,y)$. The time and space complexity is not affected.
\end{proof}











\subsection{Polylog Space algorithm}

Our algorithm recursively use the above ideas with carefully picked parameters. 

In the following, we set $b= \lceil \log n\rceil $ and $\eps = \frac{1}{b}$. We call our space-efficient approximation algorithm for edit distance \emph{SpaceEfficientApproxED} and give the pseudocode in algorithm~\ref{algo:SpaceEfficientApproxED}. %We sometimes omit floors and ceilings to improve the readability.

\begin{algorithm}[H]
	\SetAlgoLined
	\DontPrintSemicolon
	\KwIn{Two strings $x$ and $y$, integer $b$, and a small constant $\eps \in (0,1)$} 
	%\Comment*{without loss of generality, we assume $|x| \leq|y|$ }
	\If{$|x|\leq b$ \label{len}}{
		compute $\ed(x,y)$ exactly \;
		\Return{$\ed(x,y)$} \;
	}
	$ed\gets \infty$\;
	set $n = |x|$ and $m = |y|$ \;
	divide $x$ into $b$ block each of length at most $\lceil n/b \rceil$ such that $x = x^1\circ x^2 \circ \cdots \circ x^{b}$\;
	%set $\eps' =  \eps/2 $ and $\eps'' = \eps'/10$\;
	set $\eps' = \eps/10$ \;
	\ForEach{$\Delta= 0 \textbf{ or } \lceil (1+\eps)^j\rceil \textbf{ for some integer } j \text{ and } \Delta\leq \max\{n,m\}$ \label{algo:SpaceEfficientApproxEDDeltaLoop}}{
		\For{$ i = 1$ \textbf{to} $b$}{
			\ForEach{$(a,b)\in \text{CandidateSet}(n,m,(l_i,r_i),\eps',\Delta)$}{
				$M(i,(a,b))\gets \text{SpaceEfficientApproxED}(x^i, y_{[a,b]},b, \eps')$\label{algo:SpaceEfficientApproxED_recurse}\;
			}
		}
		$ed\gets \min\{ed,\text{DPEditDistance} (n,m,b,\eps', \Delta,M)\}$\;
	}
	\Return{$ed$}
	\caption{SpaceEfficientApproxED}
	\label{algo:SpaceEfficientApproxED}
\end{algorithm}

We have the following result. 

\begin{lemma}
	\label{lem:SpaceEfficientApproxED}
	Let $b = \lceil \log n\rceil $ and $\eps = \frac{1}{b}$, then $\text{SpaceEfficientApproxED} (x,y, b,\eps)$ outputs a $(1+O(\frac{1}{\log \log n}))$-approximation of $\ed(x,y)$ with $O(\log^4 n)$ bits of space in $\tilde{O}(n^7)$ time. 
\end{lemma}

\begin{proof} [Proof of Lemma~\ref{lem:SpaceEfficientApproxED}]

	Algorithm~\ref{algo:SpaceEfficientApproxED} is recursive. We start from level one and every time \emph{SpaceEfficientApproxED} is called, we enter the next level. We say the largest level we will reach is the maximum depth of recursion. In the following, to avoid ambiguity, $x$ and $y$ denote the input strings at the first level and $n$ is the length of string $x$.
	
	Notice that every time the length of first input string at $i$-th level is at most $\frac{n}{b^{i-1}}$. The recursion terminates when the length of first input string is no larger than $b$. Thus the maximum depth of recursion is at most $\log_b n \leq \log_{\log n} n= \frac{\log n}{\log \log n}$. We denote the maximum depth of recursion by $d$. 

	We first show the correctness of our algorithm by prove the following claim.
	
	
	\begin{claim}
		At the $l$-th level, the output is a $(1+ \eps)^{d-l}$ approximation of the edit distance of its input strings.
	\end{claim} 
	\begin{proof}
		We prove this by induction on $l$ from $d$ to $1$. For the base case $ l= d$, we output the exact edit distance. The claim holds trivially. 
		
		Now, we assume the claim holds for the $l+1$-th level. At the level $l$, if the input string $x$ has length no larger than $b$, we output the exact edit distance. The claim holds for level $i$. Otherwise, since we tried every $\Delta= \lceil (1+\eps)^j\rceil \text{ for some integer } j \text{ and } \Delta\leq n+m$, one of $\Delta$ satisfies $\ed(x,y)\leq\Delta\leq(1+\eps_i)\ed(x,y)$. Denote such a $\Delta$ by $\Delta_0$. Notice that $M(i,(a,b))$ is a $(1+\eps)^{d-(l+1)}$ approximation of $\ed(x^i,y_{[a,b]})$ by the inductive hypothesis. By lemma~\ref{lem:DPEditDistance}, $\text{DPEditDistance} (n,m,b,  \eps,\Delta_0, M)$ outputs a $(1+\eps)(1+\eps)^{d-(l+1)}= (1+\eps)^{d-l}$ approxiamtion of $\ed(x,y)$ when $\Delta  = \Delta_0$. This proves the claim
		
	\end{proof}
	
	By the above claim, for the first level, our algorithm always output a $(1+\eps)^{d-1}   = 1+O(\frac{1}{\log \log n})$ approximation of $\ed(x,y)$.  

	We now turn to the space and time complexity. We can consider our recursion structure as a tree. The first level corresponds to the root of the recursion tree. Notice that we need to try $O(\log_{1+\eps}(n)) = O(\log^2 n)$ different $\Delta$. For each $\Delta$, we need to query the next level $O(b(\frac{b\log n}{\eps^2})) = O(\log^5 n)$ time. This is because there are $b$ blocks and each block has $O(\frac{b\log n}{\eps^2})$ candidate intervals. Thus, the recursion tree is of degree $O(\log^7 n)$ with depth $d = O(\frac{\log n}{\log \log n})$.
	
	Running the algorithm essentially has the same order as doing a depth first search on the recursion tree. At each level of the recursion, we only need to remember the information in one node. Thus, total space required is equal to the space needed for one inner node times the depth of recursion tree, plus the space needed for one leaf node. 
	
	For the leaf nodes, the first input string is of length at most $b$, we can compute the edit distance exactly with space $O(b\log n)$ bits of space. 
	
	For other nodes, the task is to run a dynamic programing, i.e. algorithm \emph{DPEditDistance} where we need to query the next level of recursion to get the matrix $M$. In algorithm \emph{DPEditDistance}, the input is a matrix $M$ and we need to compute a matrix $A$. For matrices $A$, the rows are indexed by $i $ from $0$ to $ b$ and for the $i$-th row, the columns are indexed by the elements in set $C^i$. $C^i$ is the set of starting points of intervals in $C^i_{\eps,\Delta}$. By the proof of lemma~\ref{lem:CandidateSet}, $C^i$ is of size $O(\frac{b}{\eps})$.
	
	According to the proof of lemma~\ref{lem:DPEditDistance}, we can divide the dynamic programming into $b$ steps and for each step, we update one row of $A$. When computing the $i$-th row of $A$, we only need to query the $i-1$-th row of $A$ and the $i$-th row of $M$. Thus, the space used to remember previous rows of $A$ can be reused. Also, we only query each element in the $i$-th row of $M$ once, so we do not need to remember matrix $M$ and this does not affect the time complexity. Thus, for each inner node of the recursion, we only need space enough for storing two rows of matrix $A$ and each element of $A$ is an integer no larger than $n$. The space for each inner node is bounded by $O(\frac{b}{\eps}\log n)$ bits. 
	
	Thus, the space complexity of our algorithm is bounded by $O(d\frac{b}{\eps}\log n +  b\log n )= O(\log^4 n)$ bits.
	
	
	
	
	
	
	
	For time complexity, we denote the time used for computation at the $i$-th level by $T_i$ (excluding the time used for calling \emph{SpaceEfficientApproxED} at the $i$-level). The time complexity is bounded by the sum of time spent at each level. Denote the total running time by $T$, we have $T = \sum_{i = 1}^d T_i$.
	
	Once \emph{SpaceEffientApproxED} is called at the $(i-1)$-th level, we enter the $i$-th level. 
	
	Each time we enter the $i$-th level, there are two possible cases. For the first case, the operation at the $i$-th level is calculating the exact edit distance with one of the input string has length at most $b$ and the other string has length $O(b/\eps)$. It takes $O(\frac{b^2}{\eps})$ time. 
	
	Otherwise, we run $\text{DPEditDistance}$ for $O(\log_{1+\eps} n )= O(\frac{\log n}{\eps})$ times. By lemma~\ref{lem:DPEditDistance}, it takes $O(\frac{b^3\log n}{\eps^3})$ time. 
	
	Thus, each time we enter the $i$-th level, the time required at that level is bounded by $O(\frac{b^3\log^2 n}{\eps^4}) = O(\log^9 n)$. According to the recursion tree, we enter the $i$-th level  $O((\log^7 n)^{i-1 })$ times. Thus, $T_i = O(\log^9 n(\log^7 n)^{i-1 })$. Since $i\leq d \leq \frac{\log n}{\log \log n}$, $T_i$ is bounded by $O(\log^9 nn^7$. The total running time is bounded by $\tilde{O}(n^7)$.
	
	

	
\end{proof}











